Guarantees for Nonlinear Representation Learning: Non-identical Covariates, Dependent Data, Fewer Samples

A driving force behind the diverse applicability of modern machine learning is the ability to extract meaningful features across many sources. However, many practical domains involve data that are non-identically distributed across sources, and statistically dependent within its source, violating vital assumptions in existing theoretical studies. Toward addressing these issues, we establish statistical guarantees for learning general $\textit{nonlinear}$ representations from multiple data sources that admit different input distributions and possibly dependent data. Specifically, we study the sample-complexity of learning $T+1$ functions $f_\star^{(t)} \circ g_\star$ from a function class $\mathcal F \times \mathcal G$, where $f_\star^{(t)}$ are task specific linear functions and $g_\star$ is a shared nonlinear representation. A representation $\hat g$ is estimated using $N$ samples from each of $T$ source tasks, and a fine-tuning function $\hat f^{(0)}$ is fit using $N'$ samples from a target task passed through $\hat g$. We show that when $N \gtrsim C_{\mathrm{dep}} (\mathrm{dim}(\mathcal F) + \mathrm{C}(\mathcal G)/T)$, the excess risk of $\hat f^{(0)} \circ \hat g$ on the target task decays as $\nu_{\mathrm{div}} \big(\frac{\mathrm{dim}(\mathcal F)}{N'} + \frac{\mathrm{C}(\mathcal G)}{N T} \big)$, where $C_{\mathrm{dep}}$ denotes the effect of data dependency, $\nu_{\mathrm{div}}$ denotes an (estimatable) measure of $\textit{task-diversity}$ between the source and target tasks, and $\mathrm C(\mathcal G)$ denotes the complexity of the representation class $\mathcal G$. In particular, our analysis reveals: as the number of tasks $T$ increases, both the sample requirement and risk bound converge to that of $r$-dimensional regression as if $g_\star$ had been given, and the effect of dependency only enters the sample requirement, leaving the risk bound matching the iid setting.

==> commands.tex <==
% Definitions of handy macros can go here

\newcommand{\dataset}{{\cal D}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\e}{\varepsilon}
\DeclareMathOperator{\diam}{\textnormal{diam}}

\newcommand{\graph}{\textnormal{graph }}

\newcommand{\Prob}{\mathbf{P}}
\newcommand{\V}{\mathbf{V}}
\newcommand{\CV}{\mathbf{V}}
\newcommand{\D}{\,{\buildrel d \over =}\,}
\newcommand{\sgn}{\textnormal{sgn}}
\newcommand{\adj}{\textnormal{adj }}
\newcommand{\tildesymbol}{\textnormal{~}}

\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\spnc}{\overline{span}}
\DeclareMathOperator{\im}{im}

\DeclareMathOperator{\rel}{rel}
\DeclareMathOperator{\col}{col}

\DeclareMathOperator{\ran}{ran}
\DeclareMathOperator{\polylog}{polylog}

\DeclareMathOperator{\esup}{ess\: sup}
\DeclareMathOperator*{\infsup}{inf\: sup}

\DeclareMathOperator{\VEC}{\mathsf{vec}}
\DeclareMathOperator{\dop}{\mathsf{D}}
\DeclareMathOperator{\I}{\mathtt{I}}
\DeclareMathOperator{\J}{\mathtt{J}}
\newcommand{\diff}{\mathtt{d}}



%Theorems

\DeclareMathOperator*{\esssup}{ess\,sup}


\newcommand{\bigceil}[1]{\left\lceil #1 \right\rceil}



\newcommand{\scrA}{\mathscr{A}}
\newcommand{\scrH}{\mathscr{H}}
\newcommand{\scrF}{\mathscr{F}}
\newcommand{\scrG}{\mathscr{G}}
\newcommand{\scrP}{\mathscr{P}}
\newcommand{\sfX}{\mathsf{X}}
\newcommand{\sfY}{\mathsf{Y}}
\newcommand{\sfZ}{\mathsf{Z}}
\newcommand{\sfP}{\mathsf{P}}
\newcommand{\sfQ}{\mathsf{Q}}
\newcommand{\sfM}{\mathsf{M}}
\newcommand{\Px}{\sfP_{X}}
\newcommand{\Pz}{\sfP_{Z}}
\newcommand{\Pxy}{\sfP_{XY}}
\newcommand{\Pxbar}{\sfP_{\bar{X}}}

\newcommand{\dx}{d_{\mathsf{X}}}
\newcommand{\dgx}{d_{\scrG(\mathsf{X})}}
\newcommand{\dy}{d_{\mathsf{Y}}}
\newcommand{\dz}{d_{\mathsf{Z}}}
\newcommand{\dv}{d_{\mathsf{V}}}
\newcommand{\du}{d_{\mathsf{U}}}


\renewcommand{\Pr}{\mathbf{P}}

\newcommand{\CC}{\ensuremath{\mathscr{C}}}
\newcommand{\snorm}[1]{\ensuremath{\| #1\|}}
\newcommand{\iid}{iid}
\newcommand{\set}[1]{\ensuremath{\left\{ #1\right\}}}
\newcommand{\Gammadep}{\Gamma_{\mathsf{dep}}}
\newcommand{\matr}[1]{\ensuremath{\clint{\begin{array} #1 \end{array}}}}
\newcommand{\bigabs}[1]{\left| #1 \right|}
\newcommand{\clint}[1]{\ensuremath{\left[ #1\right]}}

%%%other commands

\newcommand{\bignorm}[1]{\left\lVert #1 \right\rVert}

\newcommand{\bigip}[2]{\ensuremath{\left\langle #1, #2 \right\rangle}}
\newcommand{\tvnorm}[1]{\| #1 \|_{\mathsf{TV}}}
\newcommand{\opnorm}[1]{\| #1 \|_{\mathsf{op}}}
\newcommand{\bigopnorm}[1]{\left\| #1 \right\|_{\mathsf{op}}}
\newcommand{\biglambda}[1]{\lambda_1\left( #1 \right)}
\newcommand{\mumin}{\underline{\mu}}
\newcommand{\grad}{\mathrm{grad}}
\newcommand{\sym}{\mathrm{sym}}


\newcommand{\Stephen}[1]{{\color{ForestGreen}stephen: #1}}
\newcommand{\Ingvar}[1]{{\color{red}ingvar: #1}}

%%%thm env
%%% I changed it to number within section.
%%% Otherwise we'd have things like "Proposition 21" which looks weird
%%% Feel free to change it back

\newtheorem{problem}{Problem}[section] % same for example numbers

\newtheorem{example}{Example}[section]


\newcommand{\blue}[1]{{\color{blue}#1}}
%\declaretheorem[name=Theorem,numberwithin=section]{theorem}
%\declaretheorem[name=Lemma,numberwithin=section]{lem}
%\declaretheorem[name=Definition,numberwithin=section]{definition}


==> icml/icml_tex/worked_examples.tex <==
\section{Examples}\label{sec: examples}

==> tex/ERM.tex <==
\subsection{Two-Stage ERM}


In the first step, we simply run empirical risk minimization over $T$ training tasks  and then proceed to extract the star estimator for $g_\star$:
\begin{equation}\label{eq:ermg}
    \begin{aligned}
        (\bar f_{1:T}, \widehat g)& \in \argmin_{(f,g)\in \scrF^{\otimes T}\times\scrG} \sum_{t=1}^T \sum_{i=1}^n \|(f,g)(X_{it})-Y_{it}\|_2^2
    \end{aligned}
\end{equation}

In the second step, we repeat the process over the samples from transfer task, for the hypothesis class $\scrF \times \{\widehat g\}$ to obtain a star-estimator for $f_0$: 
\begin{equation}\label{eq:ermf}
    \begin{aligned}
        \widehat f_0  \in \argmin_{f \in \scrF} \sum_{i=1}^m \|(f,\widehat g)(X_{0t})-Y_{0t}\|_2^2
    \end{aligned}
\end{equation}
Our final estimator of $(f_0,g_\star)$ is $(\widehat f_0, \widehat g)$ where $\widehat f_0$ is obtained from \eqref{eq:ermf} and $\widehat g$ from \eqref{eq:ermg}.



Our analysis begins with the canonical following risk decomposition:
\begin{equation*}
\begin{aligned}
    \mathtt{E}(f,g) &= \underline{\sfP} \|(f,g)(X)- Y\|_2^2 - \underline{\sfP} \|(f_{0,\star},g_\star)(X)-Y\|_2^2\\
    &=\underline{\sfP} \|(f,g)(X)- Y\|_2^2-\inf_{f\in \scrF}\underline{\sfP} \|(f,g)(X)- Y\|_2^2 \\
    &+\inf_{f\in \scrF}\underline{\sfP} \|(f,g)(X)- Y\|_2^2- \underline{\sfP} \|(f_{0,\star},g_\star)(X)-Y\|_2^2
\end{aligned}
\end{equation*}
By invoking our identifiability condition \eqref{ass:id} and applying it to the above decomposition, the following lemma is immediate.
\begin{lemma}
\label{lem:decomp}
Assume that \eqref{ass:id} holds. Then:
\begin{equation}
\label{lem:decomp:eq}
\begin{aligned}
    \mathtt{E}(\widehat f_0,\widehat g) & \leq \underline{\sfP} \|(\widehat f_0,\widehat g)(X)- Y\|_2^2-\inf_{f\in \scrF}\underline{\sfP} \|(f,\widehat g)(X)- Y\|_2^2 \\
    &+ \frac{\nu^{-1}}{T }\sum_{t=1}^T  
    \inf_{f \in \scrF} \Big(\sfP_t  \|( f ,\widehat  g)(X)- (f_{t,\star},g_\star)(X)\|_2^2\Big)\\
    &\leq \underline{\sfP} \|(\widehat f_0,\widehat g)(X)- Y\|_2^2-\inf_{f\in \scrF}\underline{\sfP} \|(f,\widehat g)(X)- Y\|_2^2 \\
    &+ \frac{\nu^{-1}}{T }\sum_{t=1}^T  \Big(\sfP_t  \|(\widehat f_t ,\widehat  g)(X)- (f_{t,\star},g_\star)(X)\|_2^2\Big)
\end{aligned}
\end{equation}
\end{lemma}

A second consequence of \eqref{ass:id} is that the noise level of the linear (first) component of \eqref{lem:decomp:eq} is $\sigma^2+o(1)$ under mild conditions.

\begin{lemma}
    \begin{equation}
        \begin{aligned}       
\inf_{f\in \scrF}\underline{\sfP} \|(f,\widehat g)(X)- Y\|_2^2 
&\leq \underline{\sfP} \|(f_{0,\star},g_\star)(X)-Y\|_2^2 +\nu^{-1}  \frac{1}{ T }\sum_{t=1}^T  \Big(\sfP_t  \|(\widehat f_t,\widehat g)(X)- (f_{t,\star},g_\star)(X)\|_2^2\Big)
        \end{aligned}
    \end{equation}
\end{lemma}

\begin{proof}
        \begin{align*}       
        \inf_{f\in \scrF}\underline{\sfP} \|(f,\widehat g)(X)- Y\|_2^2 &\leq \underline{\sfP} \|(f_{0,\star},g_\star)(X)-Y\|_2^2 +\nu^{-1}  \frac{1}{ T }\sum_{t=1}^T\inf_{f\in\scrF} \left\{  \Big(\sfP_t  \|(f,\widehat g)(X)- (f_{t,\star},g_\star)(X)\|_2^2\Big)\right\} \\
        &\leq \underline{\sfP} \|(f_{0,\star},g_\star)(X)-Y\|_2^2 +\nu^{-1}  \frac{1}{ T }\sum_{t=1}^T  \Big(\sfP_t  \|(\widehat f_t,\widehat g)(X)- (f_{t,\star},g_\star)(X)\|_2^2\Big)
        \end{align*}
\end{proof}

The key observation is that \Cref{lem:decomp} decomposes bounding the excess risk into a sum of two terms, the first of which is the excess risk of the empirical target task weight $\widehat f_0$ conditioned on $\widehat g$, and the second the task-averaged estimation error of the joint estimates $\widehat f^{(t)} \circ \widehat g$, $t \in [T]$. For a linear class $\calF$, the first term can be controlled with new techniques for non-realizable, non-iid linear regression developed in \cite{ziemann2023noise}, where the non-realizability arises from the mismatch between $\widehat g$ and $g_\star$.
% through which the covariates are passed. 
Toward addressing the second term, \cite{ziemann2022learning} provide a comprehensive toolkit for the bounding estimation errors for sequentially dependent covariates.

\red{Proof structure:
\begin{enumerate}
    \item $\beta$-mixing $\implies$ lower isometry.

    \item Lower isometry $\implies$ learning with little mixing reduction: bounding estimation error reduces to bounding martingale offset complexity.

    \item Estimation error 
    bound $\implies$ bound on noise level of misspecified LS term; can apply appropriate tools to retrieve correct variance level with mixing. 
    
\end{enumerate}
}

\begin{proposition}[Main components; informal]
    Under appropriate assumptions on the covariate distributions $\underline\sfP$, $\{\sfP^{(t)}\}_{t \in [T]}$, and function classes $\calF, \calG$, the following bounds hold:
    \begin{align}
        \underline{\sfP} \|(\widehat f_0,\widehat g)(X)- Y\|_2^2-\inf_{f\in \scrF}\underline{\sfP} \|(f,\widehat g)(X)- Y\|_2^2 \leq \red{???}
    \end{align}

    \begin{align}
        \frac{1}{T}\sum_{t=1}^T  \Big(\sfP_t  \|(\widehat f_t ,\widehat  g)(X)- (f_{t,\star},g_\star)(X)\|_2^2\Big) \leq \red{???}
    \end{align}
    \red{high prob or in exp?}
    \Ingvar{For high probability: it is easy to state bounds in terms of "offset complexity", but proving high probability bounds for the offset complexity that scale *correctly* is a little more subtle once we go beyond parametric rates (chaining a Sobolev ellipsoid does not mesh well with offset complexity, =metric entropy that scales like $ poly (1/\e)$). OTOH for bounded classes it is always easy to get in expectation bounds that scale correctly, even for large nonparametric classes. I suggest we do high probability for small classes (=metric entropy that scales like $ d\times polylog (1/\e)$) and complement with in expectation for bdd classes.}
\end{proposition}

==> tex/abstract.tex <==
\begin{abstract}
    A driving force behind the diverse applicability of modern machine learning is the ability to extract meaningful features across many sources. However, various practical domains involve data that are non-identically distributed across sources and may be statistically dependent within its source, which violate vital assumptions in existing theoretical studies. Toward addressing these issues, we provide statistical guarantees for learning general \textit{non-linear} representations from \textit{dependent} ($\beta$-mixing), \textit{non-identically distributed} data.  
    Specifically, we consider estimating $T+1$ functions $f_t \circ h$ in a function class $\calF \circ \calH$, where $f_t$ are task specific linear functions and $h$ is the shared representation. Estimation is performed using $n$ $\beta$-mixing samples from each of $T$ source tasks and $m$ $\beta$-mixing samples from a target task. The source task data is used to determine an estimate $\hat h$ for the representation, which is in turn used to estimate $\hat f_0$ for the target task. If $C(\cdot)$ denotes the complexity of a function class, then  our results show that the excess risk of the estimate $\hat f_0 \circ \hat h$ on the target task decays as $\tilde \calO \paren{\frac{C(\calH)}{nT} + \frac{C(\calF)}{m}}$. Notably, after some burn-in time, our bonds match the rates of the iid setting \emph{with no dependence on the mixing time}.
    We validate our analysis with numerical experiments performing imitation learning over non-linear dynamical systems.
    
    %We identify an interpretable task-diversity condition \Ingvar{How much should toot this---its kind of similar to trip?}, under which we recover guarantees that scale near-optimally in the number of data and sources, unifying and improving aspects of prior work. Our tools are highly modular, and thus may be of independent interest \Ingvar{what tools exactly are these?}. Lastly, we provide numerical experiments over non-linear dynamical systems to validate our analysis.
\end{abstract}

==> tex/additional_experiments.tex <==
\section{Additional Experiments}

Omitted training details and architectural choices may be found in the anonomized Github repository: \url{??}

\subsection{Building Energy Consumption Prediction} 
\Cref{fig: building energy prediction} depicts the advantages of using a shared representation for time series forecasting. The task is predicting next-day energy consumption in buildings based on the current day's data. We use energy data from 31 buildings provided by \cite{schneider2018building}, ensuring both consumption and temperature records are available for a duration ranging from several months to years. The energy data for each building is normalized between $0$ and $1$. 

The following features are used to make the predictions:
\begin{itemize}[noitemsep, nolistsep]
    \item Energy consumption and temperature from the past five days.
    \item One-hot encodings representing weekdays.
    \item A value between $0$ and $1$ indicating the time of the year.
\end{itemize}

We use a two-layer MLP (512 neurons/layer) for predictions. Building-specific models use the output directly, while the shared representation outputs a 4 dimensional feature, followed by a linear layer for task-specific predictions. The shared representation is trained on a random selection of 25 buildings, then finetuned and evaluated on the remaining six. Due to the limited data, we obtain 25 random splits of the tasks into the pretraining and target tasks. We plot the median and shade the 20\%-80\% quantiles for the resulting Root Mean Squared Error (RMSE) over all target task evaluation results. We train on variable amounts of data for the target tasks, indicated on the $x$-axis of the plot. Training is performed on the first \texttt{\# Target Task Training Data} samples from the target task. The RMSE is then evaluated for the one step ahead predictions over the remainder of the data available for the building. The networks are trained for 100 epochs using pytorch's $\texttt{adam}$ optimizer with a step size of $10^{-4}$ and weight decay of $10^{-2}$ using a batch size of $64$. Our results illustrate the benefit of leveraging the shared representation in this setting, especially in the low data regime. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{tex/figures/energy_pred_RMSE.pdf}
    \caption{Comparison of results for building energy prediction with a shared representation and without. In the low data regeime, the shared representation offers a significant benefit, which diminishes as more target task data becomes available.}
    \label{fig: building energy prediction}
\end{figure}


\subsection{Imitating a collection of expert behaviors} 

Here, we show the benefit of multi-task representation learning for imitating expert demonstrations. In particular, we consider a single dynamical system with a collection of experts which execute diverse behaviors. The system we consider is the Mujoco ant robot, depicted in \Cref{fig: mujoco ant}. The diverse behaviors are for the ant to run at different velocities. To obtain expert demonstrations, we first select 64 different desired velocities, characterized by one of eight possible speeds $0.5, 1.0, ..., 4.0$ in $m/s$, and one of eight possible directions $0^\circ, 45^\circ, \dots, 315^\circ$. Experts are trained to run at each of these velocities using Soft Actor Critic reinforcement learning by the Stable-Baselines3 project \citep{raffin2021stable}. The experts consist of Multi-Layer Perceptrons with two hidden layers of 256 units each and ReLU activations. Note that we are not enforcing the existence of a shared representation in the expert policies. Instead, we assume that such a shared representation approximately exists due to the underlying task similarity. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{tex/figures/Screenshot 2023-08-15 at 6.38.04 PM.png}
    \caption{A depiction of the Mujoco Ant Simulated Robot}
    \label{fig: mujoco ant}
\end{figure}

    
Once the experts are trained, we randomly sample $H=40$ velocities to serve as our source tasks. From these tasks, we collect $100$ trajectories. These are used to pretrain a multi-task policy. The policy is parametrized as a 3 layer MLP with hidden sizes $512\times512\times32$ and GELU activations in addition to Batch Normalization. The policy for each task is forced to share the representation, but it may select the head parameters (the final layer of weights in the network) specific to the task. Specifically, we apply stochastic gradient descent to approximate a solution to \eqref{eq:ermg}, where $Y$ are the expert actions, and $X$ is the state of the robot. The summation over $i$ denotes all of the expert data we have for a particular task, and therefore ranges over all trajectories collected from the corresponding expert controller, and all timesteps within the trajectory. 

The remaining $24$ velocities serve as target tasks. For each target task, we collect $N_{\mathrm{target}}$ trajectories\footnote{We consider various values of $N_{\mathrm{target}}$ ranging from $1$ to $30$.}. We compare three approaches to imitate the expert policy using these target datasets: target task specific behavior cloning from scratch, behavior cloning to select the network head specific to the target task using the frozen representation from the pre-training step (as in \eqref{eq:ermf}), and behavior cloning to select the network head specific to the target task in addition to finetuning the representation that was determined in the pre-training step. Finetuning is performed by running the optimizer with a stepsize on the representation parameters that is $1/10^{\mathrm{th}}$ the size of the stepsize used for the head parameters. 
  
Once the target policies are obtained, we obtain new random initializations of the robot, and roll out the learned policies, as well as the expert policies. We evaluate the input error, which is the mean squared error between the actions taken by the expert policy and the actions taken by the learned policy when both are evaluated either on the sequence of states generated by rolling out the expert policy, or the sequence of states generated by rolling out the learned policy. We also evaluate the normalized reward of the learned rollout, which is the reward of the rollout of the trained policy divided by the reward for the rollout of the expert policy. \Cref{fig: running ant comparison plots} shows these three  metrics for each of the learning approaches described above, as we vary the number of target task expert trajectories that are available to learn from. We plot the mean, and shade the standard deviation for these metrics over $50$ evaluation rollouts on each of the 24 target tasks for $10$ random seeds over the entire data collection and training process. Our results indicate illustrate that the pure representation learning (the \texttt{no\_finetune} curve) performs poorly in this setting, likely due to the absence of realizability caused by the fact that the experts themselves do not share a representation. However, this limitation can be overcome by incorporating a small amount of finetuning, in which the parameters of the shared representation are updated for the target task. Doing so results in a test loss that tends to be is lower than the that achieved by performing behavior cloning from scratch (See \Cref{fig: test loss}). However, there is higher spread in the loss representation learning approach, due to the possibility of target tasks that are more or less well aligned with the pre-trained representation. The improved test loss carries over to lower input gap between the expert and learned controller on the learned trajectory, visualized in \Cref{fig: imitation error}, as well as higher normalized reward, visualized in \Cref{fig: normalized reward}.  


\begin{figure}
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{tex/figures/test.mean_expert_imitation_err_rep_vs_no.png}
    \caption{Expert Input Error}
    \label{fig: test loss}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{tex/figures/test.mean_imitation_err_rep_vs_no.png}
    \caption{Evaluation Input Error}
    \label{fig: imitation error}
    \end{subfigure} 
    \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{tex/figures/test.normalized_reward_rep_vs_no.png}
    \caption{Normalized Reward}
    \label{fig: normalized reward}
    \end{subfigure} 
    \caption{The plots demonstrate three evaluation metrics comparing single task imitation learning with multi-task representation learning for imitation learning. The curved labeled \texttt{BC} corresponds to single task imitation learning, \texttt{no\_finetune} corresponds to multi-task representation  learning without finetuning, and \texttt{finetune} is multi-task representation learning with finetuning. \Cref{fig: test loss} shows the mean squared error between the expert and learned controllers' inputs as evaluated on the state trajectory generated by the expert controller.  \Cref{fig: imitation error} shows the mean squared error between the expert and learned controllers' inputs as evaluated on the state trajectory generated by the learned controller. \Cref{fig: normalized reward} shows the reward obtained by the learned controller divided by the reward obtained by the expert controller, where the reward is the task specific reward used to train the expert controllers.}
    \label{fig: running ant comparison plots}
\end{figure}

\subsection{Visuomotor Control: Additional details}

We consider the simulation task of balancing a pole atop a cart from visual observations, as pictured in \Cref{fig: example obs}. This experimental setup is used to demonstrate the benefit of multi-task imitation learning (compared to single task imitation learning) for a visuomotor control task. We first describe the system, and how expert policies are generated. We then provide details about the imitation learning and evaluation process. 

\paragraph{System Description:} The pole is balanced by applying a force to the cart along a track. Denoting the position of the cart by $p$ and the angle of the pole by $\theta$, the system evolves according to the following dynamics:
\begin{align*}
    u &= (M+m)(\ddot p + d_p \dot p) + m\ell ((\ddot \theta + d_\theta \dot \theta) \cos\theta - \dot \theta^2 \sin\theta), \\ 
    0 &= m((\ddot p + d_p \dot p) \cos \theta + \ell(\ddot \theta + d_\theta \dot \theta) - g\sin \theta).
\end{align*}
Here, $M$ is the mass of the cart, $m$ is the mass of the pole, $\ell$ is the length of the pole, $g$ is the acceleration due to gravity, $k_p$ is the damping coefficient for cart on the track, and $k_\theta$ is the damping coefficient for the joint of the pole with the cart. The state of this system at time $t$ is denoted $x_t = \bmat{p_t & \dot  p_t & \theta_t & \dot \theta_t}^\top$. These dynamics are discretized via an euler approximation with
stepsize $dt = 0.02$.  The discrete time dynamics will be written $x_{t+1} = f(x_t, u_t)$. We further suppose that we have a camera setup next to the track, directed towards the track and centered at the zero position of the cart. This camera gives us a partial observation of the state at any time: $o_t = \mathrm{camera}(x_t)$. \Cref{fig: example obs} is one such observation generated by the PyBullet simulator when the system is at the origin. We consider a collection of instances of this system by uniformly randomly sampling $M, m, \ell \in [0.5,3.0]\times [0.05, 0.2] \times [1.0, 2.5]$, and setting $g = 9.8$, $k_p = k_\theta  =0.4$. 

\paragraph{Expert Policy Description: } The expert has access to a (noisy) key-point extractor that maps the image observations from the camera to a vector containing the position of the cart-pole joint along the track, the position of the pole tip along the track, and the height of the pole tip above the track. This provides the two keypoints illustrated in \Cref{fig: ideal keypoints}\footnote{In our experiments, the keypoint extractor is a convolutional neural network trained on a $50000$ cartpole images from instances drawn uniformly at random with states having position $p \in [-3,3]$, $\theta \in [-\pi/3, \pi/3]$, and pole lengths $\ell \in [1,2.5]$.}. We denote this noisy observation as $\mathrm{keypoint}(o_t)$. A single keypoint extractor is used by all experts (across the parameter variations of the system), and is trained from labeled data across a variety of parameter settings. After applying the keypoint extractor to the images, the ideal measurements become a simple function of $p$ and $\theta$: they may be written $\bmat{p_t & p_t + \sin(\theta_t) \ell & \cos(\theta_t) \ell}^\top$. As such, we can construct expert controllers using the dynamics of the system by synthesizing LQG controllers\footnote{We use $Q=R=\Sigma_w=\Sigma_v=I$.} for the system linearized about the upright equilibrium point. In particular, for some particular parameter realization, indexed by $h$, the corresponding expert controller generates the force $u_t^\star$ applied to the cart at time $t$ as 
\begin{align*}
     \xi_{t+1} &= A_K^{(h)} \xi_t + B_K^{(h)} \mathrm{keypoint}\paren{\mathrm{camera}(x_t) }\\ 
    u_t^\star &=  C_K^{(h)} \xi_t + D_K^{(h)} \mathrm{keypoint}\paren{\mathrm{camera}(x_t) },
\end{align*}
where $(A_K^{(h)}, B_K^{(h)}, C_K^{(h)}, D_K^{(h)})$ are constructed from two Riccati equation solutions involving the linearized system, and $\xi_t$ is a four dimensional latent state. We assume that when the input applied is applied to the system, there is an unobserved actuation noise added. Therefore, the input applied to the system at time $t$ by the expert controller will be $u_t = u_t^\star + \eta_t$, where $\eta_t \sim\calN(0,0.5)$. 

\paragraph{Imitation Learning Policy Description: } We consider imitation learning agents that operate a short history of camera observations\footnote{We use a history of 8.}. In particular, the learning agent selects inputs as  
\begin{align*}
    \hat u_t = K_{\theta} \paren{\bmat{\mathrm{camera}(x_t) \\ \vdots \\\mathrm{camera}(x_{t-\mathrm{hist}})}}.
\end{align*}
Here $K_\theta$ is a convolutional neural network with parameters $\theta$. In the single task setting, the parameters are specific to the parameter realization for the task at hand. In the multi-task setting, the network parameters are partitioned into a shared component $\theta_{\mathrm{shared}}$ and a task specific component for the final layer, $\theta_{h}$.

\paragraph{First Stage: } The shared parameters in the multi-task setting are jointly trained on a collection of $H$ source tasks.\footnote{We consider three values of $H$: $H=5, 10, 20$.}. The dataset therefore consists of demonstrations from rollouts of the expert controllers generated for $H$ systems with different parameter realizations. Expert demonstrations are obtained from $10$ independent realizations of the actuation noise sequence for each system. The length of the rollout trajectory is $500$ steps (recalling the discretization timestep of $0.02$.)

The multi-task network is jointly trained on the entire collection of source data to minimize the loss 
\begin{align*}
    \sum_{h=1}^H \sum_{i=1}^{10} \sum_{t=1}^{500} \norm{u_t^{(h)}[i] - K_{\theta_{\mathrm{shared}}, \theta_h} \paren{\bmat{\mathrm{camera}(x_t^{(h)}[i]) \\ \vdots \\\mathrm{camera}(x_{t-\mathrm{hist}}^{(h)}[i])}}}^2
\end{align*}
over the network parameters $\theta_{\mathrm{shared}}, \theta_1, \dots, \theta_H$. The superscript $h$ on the inputs and states denotes the system index that they came from, while the argument in the brackets enumerates the $10$ expert trajectories collected from each system. To obtain an approximate minimizer to the above problem, we employ the adam optimizer using a batch size of 32, weight decay of $1e^{-3}$, and learning rate of $1e^{-3}$ with a decay factor of $0.5$ every 10 epochs for a total of 100 epochs.\footnote{Tasks are mixed together in the each batch.}

\paragraph{Second Stage: }
The second stage consists of 10 target tasks, defined by new parameter realizations for the cartpole system. We compare:
\begin{enumerate}
    \item Training a convolutional neural network for each of these tasks from scratch using the data available for the task (this is single task imitation learning).
    \item Re-using the representation trained for the collection of source tasks along with a head that is fit to the target task. The head is obtained by solving a least squares problem by computing the shared representation for the history of camera observations in the expert demonstrations and solving a regression problem to match the expert inputs. 
\end{enumerate}
For each target task, we again collect expert demonstrations. Here, we consider a variable number of trajectories, $N_{\mathrm{target}}$. Each trajectory is again obtained by rolling out the corresponding expert controller for $500$ steps under new, independent realizations of the actuation noise. These expert trajectories are used to fit a linear head for the corresponding target tasks for the multi-task setting, and to train a behavior cloning agent from scratch for the single task setting. 

\paragraph{Evaluation Results: } Once the target controllers are trained, we evaluate them by rolling them out on the cartpole system with the parameters for which they were designed. These evaluation rollouts occur by rolling out out the single-task learned, multi-task learned, and expert controller under new realizations of the actuation noise. We track the input imitation error over the entire trajectory, which is the MSE of the gap between the inputs applied by the expert, and the inputs a learned controller $\hat K$ would apply when faced with the same observations:
\[{\sum_{t=1}^{500} \norm{u_t^\star - \hat K\paren{\bmat{\mathrm{camera}(x_t^\star) \\ \vdots \\ \mathrm{camera}(x^\star_{t-\mathrm{hist}})}}}^2}.\]
We additionally track the state imitation error between the states $\hat x_t$ from rolling out the learned controller and the states $x_t^\star$ from rolling out the expert controller:
\[ {\sum_{t=1}^{500} \norm{x_t^\star - \hat x_t}^2}.\]
We also track whether the controller lasts 500 steps without allowing the pole to fall past an angle of $\pi/2$ in either direction. We plot the results for representation learning with $5$, $10$, or $20$ source tasks, in addition to single task learning. The evaluation metrics are averaged across $50$ evaluation rollouts for each target controller. In \Cref{fig: cartpole imitation learning comparisons}, the median is plotted, with the 30\%-70\% quantiles are shaded. The median and quantiles are over $10$ random seeds for the target tasks and $5$ random seeds for the parameters of the source task instances. In the low data regime, multi-task learning excels in all metrics, with increasing benefit as more source tasks are available. In the high data regime, the single task controller eventually beats out the multi-task controllers for all metrics. 


In \Cref{fig: cartpole test loss rate}, we plot the input imitation error versus the number of source tasks available for pre-training on a $\log-\log$ scale with the number of target trajectories fixed at $100$. Neglecting the component of the error that decays with the number of target trajectories, our theoretical results predict a decay in the error of $\frac{1}{H}$, or a slope of $-1$ on a $\log\log$ plot. In \Cref{fig: cartpole test loss rate}, we observe a slope of approximately $-0.8$. The discrepancy may arise for several reasons. Firstly, the empirical risk minimizer is approximated using SGD. Secondly, the number of target trajectories used for fitting the final layer of the network is not infinite, meaning that we occur some additional error in training the final layer. 

\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{tex/figures/imitation_error_rate.pdf}
    \caption{Input imitation error of the policies trained with a shared representation plotted against the number of source tasks used to train the representation on a $\log\log$ scale. The number of target trajectories used for finetuning is fixed at $100$.}
    \label{fig: cartpole test loss rate}
\end{figure}

% We may also investigate the task overlap coefficient. This investigation is performed in the Figure below. By selecting the parameters for the target task as $\ell=1.5$, $m=0.2$, and ten values of $M$ varying between $1.0$ and $5.5$. We plot the percent of stable trials for the fine-tuned multitask controller for each value of $M$. The legend highlights the task overlap condition, which is a theoretical measure of how related the controllers are between the tasks. For settings where the task overlap coefficient is higher, the task is less aligned with source tasks, and we expect the sample complexity of fitting a controller to be higher. The truncated task overlap coefficient for a task indexed $\mathrm{tar}$ is computed as
% \begin{align*}
%     \norm{ \bmat{D_K^{(\mathrm{tar})} & B_K^{(\mathrm{tar})} C_K^{(\mathrm{tar})} & \dots & B_K^{(\mathrm{tar})} \paren{A_K^{(\mathrm{tar})}}^{\mathrm{hist}-1}C_K^{(\mathrm{tar})}}
%     \bmat{D_K^{(1)} & B_K^{(1)} C_K^{(1)} & \dots & B_K^{(1)} \paren{A_K^{(1)}}^{\mathrm{hist}-1}C_K^{(1)} \\ 
%     && \vdots \\
%     D_K^{(H)} & B_K^{(H)} C_K^{(H)} & \dots & B_K^{(H)} \paren{A_K^{(H)}}^{\mathrm{hist}-1}C_K^{(H)}}^\dagger
%     }
% \end{align*}
% \begin{figure}
%     \centering
%     \includegraphics{tex/figures/multi percent stable.png}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

% {\color{red}{ Potential changes or modifications to this expertimental setup: ADD HERE!! \begin{itemize}
%     \item Plots illustrating the relationship between the task overlap coefficient and the success rate
% \end{itemize}
% }}

==> tex/assumptions.tex <==
\subsection{Assumptions}

We focus on processes that are stochastically stable in the following sense.
 
\begin{definition}
Let $Z_{1:n}$ be a stochastic process. The $\beta$-mixing coefficients of $Z$, $\beta_Z(i)$, are:
\begin{equation}\label{eq:betacoeffs}
    \beta_{Z}(i) = \sup_{t\in[n]: t+i\leq n} \E \| \sfP_{Z_{i+t}}( \cdot \mid Z_{1:t} ) - \sfP_{Z_{i+t}} \|_{\mathsf{TV}}, \quad i \in [n].
\end{equation}
\end{definition}


We will also need an identifiability condition in order to render the learning task feasible. These are typically referred to as ``task-diversity assumptions" in the literature.

\begin{assumption}
    There exists $\nu >0$ such that, for any $g \in \calG$ the following holds:
    \begin{align}\label{ass:id}\tag{\texttt{ID}}
        \begin{split}
            &\inf_{f\in \scrF} \left\{\underline{\sfP}  \|(f,g)(X)- Y\|_2^2 - \underline{\sfP} \|(f_{0,\star},g_\star)(X)-Y\|_2^2\right\}
            \\
            \leq \;&\nu^{-1}  \frac{1}{ T }\sum_{t=1}^T\inf_{f\in\scrF} \left\{  \Big(\sfP_t  \|(f,g)(X)- (f_{t,\star},g_\star)(X)\|_2^2\Big)\right\}
        \end{split}
    \end{align}
\end{assumption}
% In order to provide guarantees in terms of the excess risk \eqref{eq:excess_risk} we require that there exists $\nu >0$ such that:

\begin{remark}
While specialized to square loss, the condition \eqref{ass:id} also differs slightly from that in \citet[Definition 3]{tripuraneni2020theory}. First, we do not require realizability, and hence, we do not need to include a model mismatch term (``$\e$" in their work). Second, the right hand side of \eqref{ass:id} is specified in terms of an \emph{estimation error} and not an \emph{excess risk} as in \cite{tripuraneni2020theory}. For realizable square-loss both notions coincide. However, in our case this weakening of the condition \eqref{ass:id} matters since the estimation error is easier to lower bound than the excess risk. \Ingvar{this remark can be removed since we actually work with realizable data}
\end{remark}

In particular, toward instantiating the task-diversity condition \eqref{ass:id} downstream, we define the following lower isometry condition on the test and source measures.

\begin{definition}\label{def: task lower isometry}
    We say that the $\mu$-lower-isometry condition \eqref{ass:iso} holds if the following is true: there exists $\mu > 0$ such that for all $f,g \in \calF \times \calG$:
    \begin{align}\label{ass:iso}\tag{\texttt{ISO}}
        \underline\sfP \|(f,g) - (f^{(0)}_\star, g_\star)\|_2^2 &\leq \mu \frac{1}{T}\sum_{t=1}^T \sfP^{(t)} \|(f,g) - (f^{(t)}_\star, g_\star)\|_2^2.
    \end{align}
\end{definition}


\red{4-2 hypercontractivity?}

\Ingvar{idk. we can assume small ball instead and show that 4-2 is sufficient for small ball (I think this makes more sense since the proofs are based directly on small-ball and not on hypcon)}



==> tex/experiments.tex <==
\section{Imitation Learning Numerical Experiment}

We consider the simulation task of balancing a pole atop a cart from visual observations, as pictured in \Cref{fig: example obs}. This experimental setup is used to demonstrate the benefit of multi-task imitation learning (compared to single task imitation learning) for a visuomotor control task. A collection of systems is obtained by randomly sampling different values for the cart mass, pole mass, and pole length parameters. The learning tasks we consider are to imitate expert policies controlling this collection of systems.

We design expert policies as linear controllers of the underlying state (consisting of the cart position and velocity, and pole angular position and angular velocity) to balance the pole in the upright position. The expert estimates the state of the system from the camera observations by first applying a keypoint extractor to the camera observations to get noisy estimates of two keypoints (visualized in \Cref{fig: ideal keypoints}), and then passing these noisy estimates into a kalman filter. A common keypoint extractor is shared by all of the experts, however the controller and the filter depend on the system parameters. Actuation noise is added to the expert input when it is applied to the system.

We use demonstrations from the aforementioned expert policies to train imitation learning policies to replicate the experts. The policies are parameterized with convolutional neural networks. They take as input a history of $8$ images, and output the control action to be applied to the system. The policies are trained by solving a supervised learning problem using the expert demonstrations.

% We compare single task imitation learning with multi-task representation learning to train the policies.
Our theoretical analysis predicts that multi-task learning helps substantially in this setting. This is due to the keypoint extractor which is shared amongst all expert policies. The part that varies between expert policies is the controller and filter, which are linear maps from the keypoints to the control action. As a consequence, the decomposition into a shared complex function (the keypoint extractor) and a simple task specific map (the controller and filter) holds in this experimental setting.  

The experimental results in \Cref{fig: cartpole imitation learning comparisons} compare multi-task learning with single task learning. We consider multi-task learning using a various number of source tasks, each consisting of $10$ expert demonstrations. The $x$-axis denotes the number of demonstrations available from the target task. For single task learning, these trajectories are used to train the entire network, while for multi-task learning they are used to fit only the final layer, keeping the representation fixed from pre-training on the source tasks. Three evaluation metrics are plotted: the mean squared error in imitating the expert input, the mean squared error in tracking the expert trajectory, and the percent of trials where the controller is stabilizing. Each metric is averaged over $50$ evaluation rollouts for each controller.  We plot the median and shade 30\%-70\% quantiles for these evaluation metrics over 5 random seeds for pretraining the representation, and 10 realizations target tasks. In all metrics, multi-task learning improves over single task learning in the low data regime. The benefit is more pronounced as more tasks are available for pre-training.


\begin{figure}
    \centering
    \subfloat[Example observation]{
    \label{fig: example obs} \includegraphics[width=0.275\textwidth]{tex/figures/cropped_cartpole_image.png}}
    \subfloat[ideal keypoint extraction]{
    \label{fig: ideal keypoints}
    \includegraphics[width=0.5\textwidth]{tex/figures/Screenshot 2023-07-24 at 12.28.45 PM.png}}
    \caption{\Cref{fig: example obs} shows an example camera observation of the pybullet simulated cartpole environment. In this image, the cartpole is at the state $x = \bmat{0 & 0 & 0 & 0}^\top$. \Cref{fig: ideal keypoints} illustrates the ideal keypoints extracted from a cartpole image.}
\end{figure}



\begin{figure}
    \centering
    \subfloat[Input Imitation Error]{
        \includegraphics[width=0.3\textwidth]{tex/figures/expert_input_gap.pdf}
    }
    \subfloat[State imitation Error]{
    \includegraphics[width=0.3\textwidth]{tex/figures/imitation_error.pdf}}
    \subfloat[Percent Stable]{
    \includegraphics[width=0.3\textwidth]{tex/figures/percent_stable.pdf}}
    \caption{Three evaluation metrics comparing the performance of multi-task imitation learning with single task imitation learning: the mean squared error between the input of the learned controller and the expert controller when evaluated on the expert trajectory, the gap between the state trajectories generated by the learned and expert controllers, and the percent of trials for which the controller keeps the pole balanced for all $500$ timesteps (the dynamics are discretized such that a timestep is $0.02$ seconds). Three curves are shown for multi-task imitation learning, generated by pre-training with a different number of source tasks. In all metrics, multi-task learning improves over single task learning in the low data regime. }
    \label{fig: cartpole imitation learning comparisons}
\end{figure}


==> tex/intro.tex <==
\section{Introduction}

Motivations
\begin{itemize}
    \item In-context learning

    \item Provable benefit of learning from heterogeneous distributions

    \item Applicable to broad suite of sequential settings, opened up by generalizing to non-identical covariate distributions.

    \item \red{(manipulator) regressor form in robotics}

    \item \red{(A form of) continuous-space model-based RL under linear function approximation with unknown features (basically sysID...)}
\end{itemize}

Technical Contributions
\begin{itemize}

    \item non-IID + non-identical covariate marginals; can extend to broader dynamical systems settings. Non-trivial as both Du and Tripuraneni assume identical marginals.

    \item sharper bounds for square loss setting. Noise level of transfer learning problem is comparable to single-task after a burn-in; compare to noise level blown up to boundedness constants in Tripuraneni \red{(fact check)}.

    \item \red{Hopefully, get rid of $d_x$ burn-in per source task, or understand better why it's fundamental for ERM.}

    \item 

    
\end{itemize}


\red{To-dos:
\begin{itemize}
    \item Misc: decide on (probability) notation and clean up.

    \item Worked examples 
\end{itemize}}

\subsection{Related Work}

\paragraph{Empirical Results} task conditioned behavior cloning agents: RT-1, RT-2, X, Gato, Transporter, PerceiverActor, RVT,  video prediction \cite{han2019video}, system identification, visuomotor control \cite{srinivas2018universal}, dynamic forecasting \cite{wang2022meta}

\paragraph{Theory results} Early works providing theoretical guarantees for multi-task representation learning assume tasks are sampled i.i.d. from some underlying distribution \citep{baxter2000model, maurer2016benefit}, resulting in excess risk bounds that decay as $\tilde \calO (\frac{1}{\sqrt T} + \frac{1}{m} )$. In particular, such bounds decay with the number of source tasks, but not the total number of samples.  \cite{du2020few, tripuraneni2020theory}  overcome this limitation by introducing structural conditions on the linear predictors and covariate distributions resulting in sufficient source ``task-diversity'', thus allowing the authors to prove excess risk bounds that decay with all of the source data, $\tilde \calO(\frac{C(\calF)}{nT} + \frac{k}{m})$. 
Extensions have been made to this model to consider more general function classes for the representation, such as RKHS \citep{meunier2023nonlinear}, and to consider settings where a shared representation is only approximately satisfied, thus requiring task-specific finetuning of the representation \citep{chua2021fine}. Analysis of representations learned from multiple sources resulting from gradient based algorithms are provided by \cite{collins2023provable} for the setting of two layer multi-layer perceptrons and by \cite{thekumparampil2021sample, zhang2023meta} for the setting of linear regression. Other works have focused on actively sampling source tasks  for efficient representation learning \citep{chen2022active}. Continual learning solves problem realted to mulit-task learning in which tasks must be solved sequentially. Analyses of this setting are offered in \cite{peng2023ideal, li2022provable}. Meta learning is also related to multi-task representation learning, considers settings solving for good common initializations of parameters from which optimal values for a particular task may be found quickly using gradient descent \citep{finn2017model}. It is shown that such approaches provably learn good representations in linear settings by \cite{collins2022maml}.  Finally, multi-task analysis may be applied to analyze in-context learning, an emergent property of large language models \citep{li2023transformers}. 
%\cite{lee2021predicting} self supervised representation learning 
%: continual or lifelong learning (tasks appear sequentially)

The practical applications of multi-task representation learning for time series data has motivated theoretical studies restricted to simplified settings. The benefits of multi-task representation learning are demonstrated for reinforcement and imitation learning in an MDP setting by \cite{cheng2022provable, arora2020provable, lu2021power, agarwal2023provable, chan2023statistical}. These works make assumptions about a generative model generative model for the source tasks, thereby sidestepping the issue of dependent data that arises in these settings.  \cite{modi2021joint,zhang2023multi} \cite{modi2021joint} study system identification and imitation learning in the continuous control setting in the precense of temporally correlated data, but restrict attention to linear representations. This work in constrast studies the nonlinear representations learned from source tasks which generate temporally correlated data. 




\subsection{Problem Formulation}
\paragraph{Notation.}
Expectation (resp.\ probability) with respect to all the randomness of the underlying probability space is denoted by $\E$ (resp.\ $\Pr$). For two probability measures $\sfP$ and $\sfQ$ defined on the same probability space, their total variation is denoted $\|\sfP-\sfQ\|_{\mathsf{TV}}$. Maxima (resp.\ minima) of two numbers $a,b\in \R$ are denoted by $a\vee b =\max(a,b)$ (resp.\ $a\wedge b = \min(a,b)$). For an integer $n\in \N$, we also define the shorthand $[n] \triangleq\{1,\dots,n\}$. 



The Euclidean norm on $\mathbb{R}^{d}$ is denoted $\|\cdot\|_2$,
and the unit sphere in $\R^d$ is denoted $\mathbb{S}^{d-1}$. The standard inner product on $\R^{d}$ is denoted $\langle\cdot,\cdot\rangle$. We embed matrices $M \in \R^{d_1\times d_2}$ in Euclidean space by vectorization: $\VEC M \in \mathbb{R}^{d_1 d_2}$, where $\VEC$ is the operator that vertically stacks the columns of $M$ (from left to right and from top to bottom). For a matrix $M$, the Euclidean norm is the Frobenius norm, i.e., $\|M\|_F\triangleq \|\VEC M\|_2$. We similarly define the inner product of two matrices $M,N$ by $\langle M, N \rangle \triangleq \langle \VEC M, \VEC N\rangle $. The transpose of a matrix $M$ is denoted by $M^\top$---and if $M$ is square---$\tr M $ denotes its trace. We also write $\opnorm{M}$ for the induced $(\R^d,\|\cdot\|_2) \to (\R^d,\|\cdot\|_2)$ norm. For two symmetric matrices $M, N$, we write $M \succ N$ ($M\succeq N)$ if $M-N$ is positive (semi-)definite. If $M$ is positive semidefinite we write $\partial M \triangleq \{ x\in \R^d \mid x^\top M x =1 \}$ for the boundary of the ellipsoid induced by $M$ (note that $\mathbb{S}^{d-1}=\partial I_d$). 


\paragraph{Samples} Let $\sfP_{it}, t\in [T]$ be probability measures over a fixed sample space $\sfZ$. We are given $n$ samples from each "training task" $t$: $Z_{it} \sim \sfP_{it}, t\in [T], i\in [n]$. We consider supervised learning: the sample space decomposes into an input space $\sfX$ and and output space $\sfY$: $\sfZ = \sfX \times \sfY$ and we write $Z_{it} = (X_{it},Y_{it})$. Moreover, we are given $m$ samples from a target task distributed according to a probability measure $\sfP_0$ over $\sfZ$: $Z_i =(X_{0i},Y_{0i})\sim \sfP_{0,i}, i\in [m]$. We will abbreviate $\sfP_t = \frac{1}{n}\sum_{i=1}^n \sfP_{it}$ and  $\sfP_0 = \frac{1}{n}\sum_{i=1}^m \sfP_{0t}$. It will also be convenient to introduce $\widehat \sfP_{1:T}$ as the measure over the entire set of training tasks datapoints ($X_{it},i\in [n],t\in[T]$) and $\widehat \sfP_0$ as the empirical measure over the the test task datapoints ($X_{i0}, i \in [m]$). We will not in general assume that the $n$ (or $m$) datapoints from each task are drawn independently of each other but instead impose a weaker martingale noise condition to be made precise in the sequel !!!???.



\paragraph{Learning task and hypotheses}
Given the above samples from training and target tasks, the goal of the learner is to perform well on the target task in terms of square loss over a fixed hypothesis class $\scrH$. To enable transfer learning, we assume that the hypothesis class $\scrH$ under consideration splits into $\scrH= \scrF \times \scrG$. Let us define:
\begin{align*}
    (f_{\star, 1:t},g_\star) \in \argmin_{(f_{1:t},g) \in \scrF^{\otimes T} \times \scrG}  \sum_{t=1}^T \sfP_t \|(f_t,g)(X_t) - Y_t\|_2^2.
\end{align*}
Hence, to each task $t\in[T]$ we associate a "head" $f_{\star,t} \in \scrF$, but we enforce a shared "representation"   $g_\star\in \scrG$, which shares information across tasks. We further denote the optimal target head: $f_{0,\star}\in \argmin_{f'\in \scrF}  \sfP_0 \|(f',g_\star)-Y\|_2^2$. Note that $f_{0,\star}$ is best possible given the best shared representation $g_\star$ (which is average-optimal over training tasks).

Let us also introduce a test time probability measure $\underline{\sfP}$ over $\sfZ$. This now allows us to make precise the learning task; using our samples from both target and training tasks, we seek to find an element $(f,g) \in \scrF\times \scrG $ that renders 
the following excess risk as small as possible:
\begin{align}
\label{eq:excess_risk}
  \mathtt{E}(f,g) \triangleq  \underline{\sfP} \|(f,g)(X)- Y\|_2^2 - \underline{\sfP} \|(f_{0,\star},g_\star)(X)-Y\|_2^2.
\end{align}
Typically, we will be interested in $\underline{\sfP} = \sfP_0$. However, in certain situations a signal from $\sfP_t,t\in[T]$ may be much weaker in some directions than a signal from $\sfP_0$. This is for instance the case if $\scrP_0$ is a marginally stable linear dynamical system (LDS) and $\scrP_t,t\in[T]$ are strictly stable LDS. In this case, recovery may still be possible against a weaker loss measure such as parameter recovery (as opposed to excess risk or prediction error under $\sfP_0$), which is captured in (bi-)linear regression by specifying an isotropic design under $\underline{\sfP}$. While our choice of $\underline{\sfP}$ is relatively free, we will require $f_{0,\star}$ to be optimal for it in the sense that $\underline {\sfP} \langle (f,g)-(f_{0,\star},g_\star), (f_{0,\star},g_\star) -Y\rangle \leq 0$ for all $(f,g) \in \scrF\times \scrG$. This can trivially be guaranteed if $Y =(f_0,g_\star)(X)$ under $\underline{\sfP}$. \textcolor{red}{FIRST TIME REALIZABILITY ISSUE ARISES IS HERE!}

==> tex/lowertail.tex <==
\section{The Lower Tail}
\label{sec:lowertail}

In this section we establish control of the form 
\begin{equation}\label{eq:loweruniformcomp}
    \frac{1}{ T }\sum_{t=1}^T \sfP_t  \|(f,g)(X)\|_2^2\lesssim \frac{1}{ nT }\sum_{t=1}^T \sum_{i=1}^{n} \|(f_t,g)(X_{t,i})\|_2^2 \quad \forall f,g\in(\scrF^{\otimes T}\times\scrG)_\star
\end{equation}
and then also
\begin{equation}\label{eq:loweruniformcond}
   \underline{\sfP}  \|(f,\widehat g)(X)\|_2^2 \lesssim \frac{1}{ n }\sum_{i=1}^{n} \|(f,\widehat g)(X_{0,i})\|_2^2 \quad \forall f\in \scrF-\{\widehat{f}_{\star|\widehat g}\}.
\end{equation}


Let us now abstract slightly and establish inequalities of the form \eqref{eq:loweruniformcomp} and \eqref{eq:loweruniformcond} for a general class of functions $\scrH$ with domain $\mathbb{R}^{\dz}$ and an arbitrary $\beta$-mixing sequence $Z_{1:n}$ taking values in $\mathbb{R}^{\dz}$. The specific cases \eqref{eq:loweruniformcomp} and \eqref{eq:loweruniformcond} will then be derived as corollaries to the general lower uniform estimate in \Cref{thm:smallballgeneral}.


To this end we partition $[n]$ into $2m$ consecutive intervals, denoted $a_j$ for $j \in [2m]$, so that $\sum_{j=1}^{2m} |a_j| = n$. Denote further by $O$ (resp. by $E$) the union of the oddly (resp. evenly) indexed subsets of $[n]$. We further abuse notation by writing $\beta_Z(a_i) = \beta_Z(|a_i|)$ in the sequel.

We split the process $Z_{1:n}$ as:
\begin{equation}\label{eq:blockstructure}
    Z^o_{1:|O|} \triangleq (Z_{a_1},\dots,Z_{a_{2m-1}}), \quad Z^e_{1:|E|} \triangleq (Z_{a_2},\dots,Z_{a_{2m}}).
\end{equation}
Let $\tilde Z^o_{1:|O|}$ and $\tilde Z^e_{1:|E|}$ be blockwise decoupled versions of \eqref{eq:blockstructure}. That is we posit that $\tilde Z^o_{1:|O|} \sim \sfP_{\tilde Z^o_{1:|O|}}$ and $\tilde Z^e_{1:|E|} \sim \sfP_{\tilde Z^e_{1:|E|}}$, where:
\begin{equation}\label{eq:blocktensor}
    \sfP_{\tilde Z^o_{1:|O|}} \triangleq \sfP_{Z_{a_1}} \otimes \sfP_{Z_{a_3}}\otimes  \dots \otimes \sfP_{Z_{a_{2m-1}}} 
    \quad \textnormal{and}\quad
    \sfP_{\tilde Z^e_{1:|E|}} \triangleq \sfP_{Z_{a_2}} \otimes \sfP_{Z_{a_4}} \otimes\dots \otimes \sfP_{Z_{a_{2m}}}.
\end{equation}
The process $\tilde Z_{1:n}$ with the same marginals as $\tilde Z^o_{1:|O|}$ and $\tilde Z^e_{1:|E|}$ is said to be the decoupled version of $Z_{1:n}$. To be clear: $\sfP_{\tilde Z_{1:n}} \triangleq \sfP_{Z_{a_1}} \otimes \sfP_{Z_{a_2}}\otimes  \dots \otimes \sfP_{Z_{a_{2m}}}$, so that $\tilde Z^o_{1:|O|}$ and $\tilde Z^e_{1:|E|}$ are alternatingly embedded in  $\tilde Z_{1:n}$. The following result is key---by skipping every other block, $\tilde Z_{1:n}$ may be used in place of $Z_{1:n}$ for evaluating scalar functions at the cost of an additive mixing-time-related term.

\begin{proposition}[Lemma 2.6 in \cite{yu1994mixing}; Proposition 1 in \cite{kuznetsov2017generalization}]
\label{prop:decoupling}
Fix a $\beta$-mixing process $Z_{1:n}$ and let $\tilde Z_{1:n}$ be its decoupled version.  For any measurable function $f$ of $Z^o_{1:|O|}$ (resp.\ $g$ of $Z^e_{1:|E|}$)
with joint range $[0,1]$ we have that:
\begin{equation}
    \begin{aligned}
        | \E(f(Z^o_{1:|O|})) - \E (f(\tilde Z^o_{1:|O|})) | &\leq \sum_{i \in E\setminus \{2m\}} \beta_Z(a_i),\\
        | \E(g(Z^e_{1:|E|})) - \E (g(\tilde Z^e_{1:|E|})) | &\leq \sum_{i \in O\setminus\{1\}} \beta_Z(a_i).
    \end{aligned}
\end{equation}
\end{proposition}


let us now define the following Rademacher average:
\begin{equation}
    \mathcal{R}(\scrH,\sfP_{\tilde Z}) =  \E \sup_{h\in \scrH} \frac{1}{n} \sum_{i =1}^n \eta_i h(\tilde Z_i) 
\end{equation}
where $\eta_{1:n}$ are Rademacher random variables independent of all other randomness. Let us further introduce the following small-ball quantity: 
\begin{equation}
    \mathcal{Q}(\scrH,\sfP_Z,u) = \inf_{h\in \scrH}\mathbf{P}_Z(h^2(Z)\geq u^2) \quad \textnormal{with} \quad  \sfP_{Z}=\frac{1}{n} \sum_{i=1}^n\sfP_{Z_i}
\end{equation}

\begin{remark}[Sufficiency of Trajectory-Hypercontractivity]
    It is straightforward to verify by Paley-Zygmund that a nontrivial estimate on $\mathcal{Q}(\scrH,\sfP_Z,u) $ only depending on $C$ can be obtained if the so-called trajectory-hypercontractivity assumption of \cite{ziemann2022learning} holds:
    \begin{equation}\label{eq:trajhypinremark}
        \frac{1}{n} \sum_{i=1}^n \E h^4(Z_i) \leq C^2 \left(\frac{1}{n} \sum_{i=1}^n \E h^2(Z_i)\right)^2 \qquad \forall h\in \scrH
    \end{equation}
    since this is again equivalent to the equivalence of the $L^4(\sfP_Z)$- and $L^2(\sfP_Z)$-norms.
\end{remark}


\begin{proposition}
    Suppose that \eqref{eq:trajhypinremark} holds. For any function class$\scrH  $ we have that:
    \begin{equation}
        \mathcal{Q}(\scrH\cap rS_{L^2},Z_{1:n},u)\geq 
    \end{equation}
\end{proposition}

\begin{proof}
    Let $h \in \scrH$ be such that $\E h^2 = r^2$. Paley Zygmund applied $h^2$ informs us that for any $\theta \in [0,1] $:
    \begin{equation}
        \begin{aligned}
            \mathbb{P} \left( h^2 > \theta r^2 \right) &\geq (1-\theta^2) \frac{(\E h^2)^2}{\E h^4}\\
            &\geq (1-\theta^2) C^2 && (\textnormal{by \eqref{eq:trajhypinremark}})\\
            &= \left(1-\frac{r^4}{u^4} \right)C^2
        \end{aligned}
    \end{equation}
\end{proof}


With these definitions in place we are poised to state a general lower uniform estimate that will be instantiated several times in the sequel.
\begin{theorem}[Blocked Theorem 2.1 of \cite{koltchinskii2015bounding} ]
\label{thm:smallballgeneral} 
Fix $\tau>0$, a consecutive partition $a_{1:2m}$ of $[n]$, and a class $\scrH$ with $\mathcal{Q}(\scrH,Z_{1:n},2\tau)>0$. Then as long as:
\begin{equation}\label{eq:burninsmallballgeneral}
   \sqrt{\max_{j\in [2m]} |a_j|}  \mathcal{R}(\scrH,\sfP_{\tilde Z}) \leq \frac{\tau \mathcal{Q}(\scrH,\sfP_Z,2\tau)}{64}
\end{equation}
we have that
\begin{equation}
    \Pr\left(\exists h \in \scrH: \frac{1}{n}\sum_{i=1}^n h^2(Z_i) < \frac{\tau \mathcal{Q}(\scrH,\sfP_Z,2\tau)}{2}   \right) \leq 4\exp\left(- \frac{n \mathcal{Q}(\scrH,\sfP_Z,2\tau)}{64\max_{j\in [2m]} |a_j|}\right)+\sum_{i=2}^{2m-1} \beta_Z(a_i)
\end{equation}
\end{theorem}

\begin{corollary}[Lower Uniform Estimate for the Composite Class]

    
    Fix $\tau>0$  and $T$ consecutive partition $a_{t,1:2m}$ of $[n]$. Let $X_{t, 1:n}$ be $T$ sequences of $\beta$-mixing random variables taking values in $\R^{\dx}$. Then as long as for every $t\in [t]$:
    \begin{equation}
   \sqrt{\max_{j\in [2m]} |a_j|}  \mathcal{R}((\scrF\times\scrG)_\star,\sfP_{t,\tilde X}) \leq \frac{\tau \mathcal{Q}((\scrF\times\scrG)_\star,\sfP_{t},2\tau)}{64}
\end{equation}
we have that
\begin{multline}
    \Pr\left(\exists (f_{1:T},g) \in (\scrF^{\otimes T}\times\scrG)_\star: \frac{1}{ nT }\sum_{t=1}^T \sum_{i=1}^{n} \|(f_t,g)(X_{t,i})\|_2^2 <\frac{1}{T}\sum_{t=1}^T \frac{\tau \mathcal{Q}((\scrF\times\scrG)_\star,\sfP_t,2\tau)}{2n}   \sum_{i=1}^{n}\E \|(f_t,g)(X_{t,i})\|_2^2 \right) \\
    %
    \leq \sum_{t=1}^T\left[ 4\exp\left(- \frac{n \mathcal{Q}((\scrF\times\scrG)_\star,\sfP_t,2\tau)}{64\max_{j\in [2m]} |a_{t,j}|}\right)+\sum_{i=2}^{2m-1} \beta_Z(a_{t,i})\right]
\end{multline}
\end{corollary}

\Ingvar{This first corollary replaces the lower uniform law in \cite{ziemann2022learning} and is aimed to control the realizable many-task component}

\Ingvar{I am not sure if the burn-in in $\mathcal{R}((\scrF\times\scrG)_\star,\sfP_{t,\tilde X})$ is optimal. Although, if $(\scrF\times\scrG)_\star = \partial \Sigma_X$ (with the obvious identification of linear functionals) then this burn-in is basically $n \gtrsim \dx$ which matches the SSD paper (ignoring $log T$ factors which appear due union bounds in both cases)}


\begin{corollary}[Lower Uniform Estimate for the Conditionally Linear Class]
    Fix $\tau>0$  and a consecutive partition $a_{1:2m}$ of $[n]$. Let $X_{1:n}$ be a sequence of $\beta$-mixing random variables taking values in $\R^{\dx}$ and a function $g : \mathbb{R}^{\dx} \to \mathbb{R}^{\dgx} $. Identify $\partial \Sigma_{g(X)} = \{ \langle v, g(\cdot) \rangle : v \in \partial \Sigma_{g(X)} \} $ and assume that
    \begin{equation}
         \sqrt{\max_{j\in [2m]} |a_j|}  \mathcal{R}(\partial \Sigma_{g(X)},\sfP_{g(\tilde X)}) \leq \frac{\tau \mathcal{Q}(\partial \Sigma_{g(X)},\sfP_{g(X)},2\tau)}{64}.
    \end{equation}
    We have that:
    \begin{multline}
    \Pr\left(\exists v \in \R^{\dgx}: \frac{1}{n}\sum_{i=1}^n \langle v,[g(X_i)g^\top(X_i) ]v \rangle  < \frac{\tau \mathcal{Q}(\partial \Sigma_{g(X)},\sfP_{g(X)},2\tau)}{2n}\sum_{i=1}^n \E \langle  v,[g(X_i)g^\top(X_i) ]v \rangle   \right) \\
    \leq  4\exp\left( -\frac{n \mathcal{Q}(\partial \Sigma_{g(X)},\sfP_{g(X)},2\tau)}{64\max_{j\in [2m]} |a_j|}\right)+\sum_{i=2}^{2m-1} \beta_X(a_i)
\end{multline}
\end{corollary}

\Ingvar{
    This second corollary replaces Theorem 4.3 of \cite{ziemann2023noise} and the rest of the nonrealizable linear regression analysis follows mutatis mutandis.
}



\subsection{Proof of \Cref{thm:smallballgeneral}}
Clearly by Markov's Inequality applied to the empirical measure and by definition of $\mathcal{Q}(\scrH,Z_{1:n},u)$:
\begin{equation}
\begin{aligned}
    \frac{1}{n}\sum_{i=1}^n h^2(Z_i) &\geq \frac{1}{n}\sum_{i=1}^n  u^2 \mathbf{1}_{h^2(Z_i)\geq u^2}\\
    %
    &
    =
    u^2\left(\mathbf{P}_Z(h^2(Z)\geq u^2) + \frac{1}{n}\sum_{i=1}^n   \mathbf{1}_{h^2(Z_i)\geq u^2}-\mathbf{P}_Z(h^2(Z)\geq 2u^2)\right)\\
    %
    &
    \geq 
     u^2\mathcal{Q}(\scrH,Z_{1:n},u)+  u^2\left( \frac{1}{n}\sum_{i=1}^n   \mathbf{1}_{h^2(Z_i)\geq u^2}-\mathbf{P}_Z(h^2(Z)\geq 4u^2)\right).
    \end{aligned}
\end{equation}

It remains to control the empirical process $ \frac{1}{n}\sum_{i=1}^n   \mathbf{1}_{h^2(Z_i)\geq u^2}-\mathbf{P}_Z(h^2(Z)\geq 4u^2)$.


Let us now define the approximate indicators $\phi_u$:
\begin{equation}
    \phi_u (s)= \begin{cases}
        1 &  s \geq 2u,\\
        \frac{s}{u} -1 & u \leq s < 2u,\\
        0 & 0 \leq s <u.
    \end{cases}
\end{equation}

It is immediate that
\begin{equation}
\begin{aligned}
  \frac{1}{n}\sum_{i=1}^n   \mathbf{1}_{h^2(Z_i)\geq u}-\mathbf{P}_Z(h^2(Z)\geq 2u) &\leq  \frac{1}{n}\sum_{i=1}^n   \phi_u[h^2(Z_i)]-\mathbf{E}\phi_u[h^2(Z_i)] \\
  %
  &
  \leq
  \sup_{h\in \scrH} \frac{1}{n}\sum_{i=1}^n   \phi_u[h^2(Z_i)]-\mathbf{E}\phi_u[h^2(Z_i)]\\
  &
  \leq 
  \sum_{\sgn \in \{O,E\}}\sup_{h\in \scrH} \frac{1}{n}\sum_{i\in \sgn}  \phi_u[|h(Z_i)|]-\mathbf{E}\phi_u[|h(Z_i)|].
\end{aligned}
\end{equation}

\paragraph{Controlling the empirical process}
Let us now control the empirical process above. We pass by the decoupled process $\tilde Z_{1:n}$. Observe that for $\sgn \in \{O,E\}$ with probability $1-2\exp(-\frac{  x^2}{\max_{j\in [2m]}|a_j|})$
\begin{equation}
\begin{aligned}
    \sup_{h\in \scrH}\frac{1}{n}\sum_{i\in \sgn}  \phi_u[|h(\tilde Z_i)|]-\mathbf{E}\phi_u[|h(\tilde Z_i)|] &=  \sup_{h\in \scrH}\frac{1}{n} \sum_{j\in 2m, a_j \subset\sgn } \sum_{i\in a_j}  \phi_u[|h(\tilde Z_i)|]-\mathbf{E}\phi_u[|h(\tilde Z_i)|]\\
    &
    %
    \leq  
     \E \sup_{h\in \scrH}\frac{4 }{n} \sum_{j\in 2m, a_j \subset\sgn }\eta_j \sum_{i\in a_j}  \phi_u[|h(\tilde Z_i)|]-\mathbf{E}\phi_u[|h(\tilde Z_i)|] + \frac{x}{\sqrt{n}}
\end{aligned}
\end{equation}
by McDiarmid's Inequality and the Giné-Zinn Symmetrization Theorem. The Ledoux-Talagrand Vector-Contraction Inequality now yields that on the same event:
\begin{equation}
\begin{aligned}
     &\sup_{h\in \scrH}\frac{1}{n}\sum_{i\in \sgn}  \phi_u[|h(\tilde Z_i)|]-\mathbf{E}\phi_u[|h(\tilde Z_i)|]\\
     &
     \leq \frac{8 \sqrt{\max_{j\in [2m]} |a_j|} }{n u} \E \sup_{h\in \scrH}\sum_{i\in \sgn} \eta_i h(\tilde Z_i) + \frac{x}{\sqrt{n}}\\
     &
     %
      \leq \frac{8 \sqrt{\max_{j\in [2m]} |a_j|} }{u} \mathcal{R}(\scrH,\sfP_{\tilde Z}) + \frac{x}{\sqrt{n}} \\
      &
      %
       \leq \frac{\mathcal{Q}(\scrH,Z_{1:n},2\tau)}{8}  + \frac{x}{\sqrt{n}} && (u=\tau \textnormal{ and } \eqref{eq:burninsmallballgeneral})\\
       &
       %
        \leq \frac{\mathcal{Q}(\scrH,Z_{1:n},2\tau)}{4} && (x=\sqrt{n}\mathcal{Q}(\scrH,Z_{1:n},2\tau)  /8 ).
\end{aligned}
\end{equation}
Consequently, by invoking \Cref{prop:decoupling} to convert the bound on $\tilde Z$-process to the $Z$-process and combining with the above, we have that with probability at least 
\begin{equation}
1 - 4\exp\left( \frac{n \mathcal{Q}(\scrH,Z_{1:n},2\tau)}{64\max_{j\in [2m]} |a_j|}\right)-\sum_{i=2}^{2m-1} \beta_Z(a_i)
\end{equation}
we have that
\begin{equation}
      \frac{1}{n}\sum_{i=1}^n h^2(Z_i) \geq \frac{\tau^2  \mathcal{Q}(\scrH,Z_{1:n},2\tau)}{2}
\end{equation}
uniformly in $h$.



==> tex/mainresult.tex <==
\section{Main Results}\label{sec: main results}

\subsection{Warm-up: Independent Covariates and Finite Representation Classes}\label{ssec: warmup}

We first consider a basic setting where the representation function class is finite $\abs{\calG} < \infty$, and covariates within each task are iid.

To reduce bounding the population risk to bounding the empirical risk, we appeal to a lower uniform argument on the representation class $\calG$, such that for each task $t \in [T]$ and a given $g \in \calG$:
\begin{equation*}
    \Sigmat_g := \Et\brac{g(x)g(x)^\top} \precsim \frac{1}{N} \sum_{i=1}^N g(\xit) g(\xit)^\top =: \hatSigmat_{g,N}.
\end{equation*}

\red{stitch uniform estimate stuff here} In particular, instantiated for independent covariates, we have

\begin{proposition}
    Fix $\tau > 0$, $g \in \calG$, and a task $t \in [T]$. Let $\xit$, $i\in[N]$ be a sequence of independent samples from $\Pt$. We identify $\partial \Sigmat_g := \scurly{\ip{v, g(\cdot)}: v \in \bbS^{r - 1}}$. As long as $N$ is large enough such that
    \begin{align}
        \calR_N(\partial \Sigmat_g, \Pt) \leq \frac{\tau}{64}\calQ(\Sigmat_g, \Pt, 2\tau) =: \frac{\tau}{64} \sbconstt{g, 2\tau},
    \end{align}
    we have the following:
    \begin{align*}
        % &\Pt\brac{\exists v \in \R^{r}: v^\top \paren{\frac{1}{N} \sum_{i=1}^N g(\xit)g(\xit)^\top }v \leq \frac{\tau \sbconstt{g, 2\tau}}{2N} v^\top \sum_{i=1}^N \Et\brac{g(\xit)g(\xit)^\top} v } \\
        &\Pt\brac{\exists v \in \R^{r}: v^\top \hatSigmat_{g,N} v \leq \frac{\tau \sbconstt{g, 2\tau}}{2} v^\top \Sigmat_g v } \leq 4\exp\paren{-\frac{N\sbconstt{g, 2\tau}}{64}}.
    \end{align*}
\end{proposition}
By union bounding over tasks $t$, we know that with high probability, the empirical covariance (passed through $g$) dominates the population in the L\"owner order, adjusted by the small-ball constant:
\begin{align}\label{eq: small ball dominance}
        \frac{1}{N} \sumN g(\xit) g(\xit)^\top \succsim \frac{\tau \sbconstt{g, 2\tau}}{2} \Et\brac{g(x)g(x)^\top}, \quad \forall t \in [T].
\end{align}
The L\"owner ordering holds when multiplying any matrix $\Ft'$ on both sides of \Cref{eq: small ball dominance} for each $t \in [T]$. Therefore, taking the trace of \Cref{eq: small ball dominance} and averaging across $t$, we get the following lower uniform bound.
\begin{corollary}\label{cor: small ball over tasks}
    Fix $\tau > 0$, $g \in \calG$. As long as $N$ is large enough such that
    \begin{align}\label{eq: small ball burn-in}
        \calR_N(\partial \Sigmat_g, \Pt) \leq \frac{\tau}{64}\sbconstt{g, 2\tau} \quad \forall t \in [T],
    \end{align}
    we have that with probability greater than $1 - 4\sum_t \exp\paren{-N\sbconstt{g, 2\tau}/64}$, for any $\scurly{\Ft} \subset \R^{d_y \times r}$,
    \begin{align*}
        % \frac{1}{N} \sumN g(\xit) g(\xit)^\top \succsim \frac{\calQ(\Sigmat_g, \Pt, 2\tau)}{2N} \sum_{i=1}^N \Et\brac{g(\xit)g(\xit)^\top}, \quad \forall t \in [T],
        \frac{1}{TN} \sumT \sumN \norm{\Ft g(\xit)}_2^2 &\geq \frac{1}{2T} \sumT \tau\sbconstt{g, 2\tau} \Et \norm{\Ft g(x)}_2^2 \\
        &\geq \frac{\tau\sbconstmin{g, 2\tau}}{2T} \sumT \Et \norm{\Ft g(x)}_2^2,
    \end{align*}
    where $\sbconstmin{g, 2\tau}:= \min_t \sbconstt{g, 2\tau}$.
\end{corollary}
Thus, we have reduced bounding the population estimation error to the empirical one, at the overhead of a per-task burn-in cost \eqref{eq: small ball burn-in}, and a small-ball constant $\sbconstmin{g, 2\tau}$.

\begin{remark}[Instantiating linear representations]
    To understand how our assumptions compare to prior work, we instantiate the linear case $\calG := \scurly{g: g(x) = Gx,\;G\in \R^{r \times d_x}}$ as considered in, e.g., \cite{du2020few, tripuraneni2020theory}. 
\end{remark}

\begin{remark}
    
\end{remark}

Now, plugging in $\Ft' = $By a standard application of the basic inequality (e.g.\ \cite{liang2015learning, ziemann2022single, ziemann2022learning}), we may bound the (task-averaged) estimation error of the empirical risk estimator by
\begin{align*}
    &\frac{1}{TN}\sumT\sumN\norm{(\fthat, \hatg)(\xit) - (\ft, g)(\xit)}_2^2 \\
    \leq \;&\frac{1}{TN} \sup_{\substack{\scurly{\ft}_{t=1}^{T} \subset \calF^{\otimes T}\\
    g \in \calG}} \sumT\sumN 4 \ip{\wit, \ft\circ g(\xit)} - \norm{\ft \circ g(\xit)}_2^2.
\end{align*}
Applying existing analyses individually on each task intuitively yields suboptimal guarantees, due to the redundancy of $\calG$ across tasks. Therefore, we take a little more care in handling the above stochastic process.
Noting $\calF \subset \R^{d_y \times r}$ is a linear class, the last line may be equivalently written as
\begin{align*}
    \frac{1}{TN} \max_{g \in \calG} \sumT \sup_{\Ft \in \calF} \sumN 4 \ip{\wit, \Ft g(\xit)} - \norm{\Ft g(\xit)}_2^2.
\end{align*}
For a given $g$, the analysis of the above process reduces to that of linear predictors.
\begin{lemma}\label{lem: linear offset basic to projection}
    For size-conforming matrices $W, Z$, with $Z$ full-rank, the following equality holds:
    \begin{align*}
        \sup_{F} \ip{W, ZF^\top} - \norm{ZF^\top}_F^2 &= \norm{(Z^\top Z)^{-1/2} Z^\top W}_F^2.
    \end{align*}
\end{lemma}
Applying \Cref{lem: linear offset basic to projection} yields:
\begin{align*}
    \sumT \sup_{\Ft \in \calF} \sumN 4 \ip{\wit, \Ft g(\xit)} - \norm{\Ft g(\xit)}_2^2 &= \sumT \norm{\paren{g(\bXt)^\top g(\bXt)}^{-1/2} g(\bXt)^\top \bWt}_F^2.
\end{align*}
We note the right hand side is precisely a sum of self-normalized martingales, which we may analyze with established tools, e.g.\ in \cite{pena2009self, abbasiyadkori2011selfnormalized, tu2022learning, ziemann2023tutorial}. This leads to the following result.
\begin{proposition}\label{prop: est error -> offset basic -> SNM}
    Fix $\tau > 0$, and let $\abs{\calG} < \infty$. Let \red{$g$ small ball assumption} and take the quantities defined therein. Then, assuming that $N$ is large enough such that
    \begin{align*}
        \calR_N(\partial \Sigmat_g, \Pt) \leq \frac{\tau}{64}\sbconstt{g, 2\tau} \quad \forall t \in [T],\;g \in \calG,
    \end{align*}
    we have the following bound on the population estimation error with probability greater than $1 - \delta$
    \begin{align*}
        \frac{1}{T}\sumT\Et\norm{\Fthat\hatg(x) - \Ftstar g_\star(x)}_2^2 &\leq \red{\#}
    \end{align*}
    
\end{proposition}

\textit{Proof of \Cref{prop: est error -> offset basic -> SNM}:} from \Cref{cor: small ball over tasks}, given ERM weights and representation $(\scurly{\Fthat}, \hatg)$ we may bound the task-wise population estimation error by its empirical counterpart \red{(change burn-in depending on how it shakes out)}, after which we apply the basic inequality \Cref{lem: linear offset basic to projection}:
\begin{align*}
    \frac{1}{T}\sumT  \Et \norm{\Fthat \hatg(x) - \Ftstar g_\star(x)}_2^2 &\leq \frac{2}{\tau\sbconstmin{g, 2\tau}} \frac{1}{TN} \sumT \sumN \norm{\Fthat \hatg(\xit) - \Ftstar g_\star(\xit)}_2^2 \\
    &\leq \frac{2}{\tau\sbconstmin{g, 2\tau}}
    \frac{1}{TN} \sup_{\substack{\scurly{\ft}_{t=1}^{T} \subset \calF^{\otimes T}\\
    g \in \calG}} \sumT\sumN 4 \ip{\wit, \ft\circ g(\xit)} - \norm{\ft \circ g(\xit)}_2^2 \\
    &\leq \frac{2}{\tau\sbconstmin{g, 2\tau}} \max_{g \in \calG} \frac{1}{TN} \sumT \norm{\paren{g(\bXt)^\top g(\bXt)}^{-1/2} g(\bXt)^\top \bWt}_F^2.
\end{align*}
To bound the self-normalized martingales on the last line, we adapt prior Frobenius norm bounds (e.g.\ \citet[Theorem 4.1]{ziemann2023tutorial} or \citet[Theorem 3.4]{abbasi2013online}) and tensorization due to independent tasks to yield the following result.
\begin{proposition}[Multi-task Frobenius-norm SNM bound]\label{prop: multi-task SNM bound}
    For each $t \in [T]$, let $\scurly{\scrF^{(t)}_i}_{i=0}^N$ be a filtration such that $\scurly{\xit}_{i=1}^N$ is adapted to $\scurly{\scrF^{(t)}_{i-1}}_{i=1}^N$ and $\scurly{\wit}_{i=1}^N$ is adapted to $\scurly{\scrF^{(t)}_i}_{i=1}^N$. Suppose that for all $i \in [N]$, $\wit$ is $\sigma^2$-conditionally sub-Gaussian with respect to $\scrF^{(t)}_i$. Assume $\xit,\wit$ are supported on $\R^d$, and let $\Sigma \in \R^{d\times d}$ be a positive-definite matrix. Then, with probability at least $1 - \delta$,
    \begin{align}
    \sumT \norm{\sumN \wit \xit^\top \paren{\Sigma + \sumN \xit\xit^\top}^{-1/2}}^2_F &\leq \sumT \brac{d \sigma^2 \log\paren{\frac{\det \paren{\Sigma + \sumT \xit\xit^\top}}{\det\paren{\Sigma}}}} + 2\sigma^2 \log(1/\delta).
    \end{align}
\end{proposition}
We note that the confidence term $2\sigma^2 \log(1/\delta)$ crucially lies outside of the summation over $T$. The proof follows from a combination of \citet[Theorem 3.4]{abbasi2013online} and a tensorization argument (see \citet[Prop.\ B.1]{zhang2023multi}) over tasks $t \in [T]$, which are by definition independent, summarized below.

\textit{Proof of \Cref{prop: multi-task SNM bound}:} a key intermediate result in the proofs of \citet[Theorem 3.4]{abbasi2013online} and \citet[Prop.\ B.1]{zhang2023multi} can be stated as the following in our context: for each $t \in [T]$, we have
\begin{align*}
    \Et \brac{\paren{\frac{\det(\Sigma)}{\det(\Sigma + \bXt^\top \bXt) } }^{d/2} \exp\paren{\frac{1}{2}\norm{(\Sigma + \bXt^\top \bXt)^{-1/2}\bXt^\top \bWt}_F^2  } } \leq 1.
\end{align*}
Importantly, since data is independent across tasks $t \in [T]$, using the above in an Markov/Chernoff inequality gets the following: defining $\barSigmaxt := \Sigma + \bXt^\top \bXt$,
\begin{align*}
    &\Prob\brac{\sumT \norm{\barSigmaxt^{-1/2}\bXt^\top \bWt}_F^2 > 2\paren{\sumT \log\paren{\frac{\det(\barSigmaxt)^{d/2} }{\det(\Sigma)^{d/2}} } + \log(1/\delta)}} \\
    =\;& \Prob\brac{\prodT \exp\paren{\frac{1}{2}\norm{\barSigmaxt^{-1/2}\bXt^\top \bWt}_F^2} > \frac{1}{\delta} \prodT
    \paren{\frac{\det(\barSigmaxt) }{\det(\Sigma)} }^{d/2}} \\
    =\; & \Prob\brac{\prodT \exp\paren{\frac{1}{2}\norm{\barSigmaxt^{-1/2}\bXt^\top \bWt}_F^2}
    \paren{\frac{\det(\Sigma)}{\det(\barSigmaxt) } }^{d/2} > \frac{1}{\delta}} \\
    \leq \;& \delta \cdot \E\brac{\prodT \exp\paren{\frac{1}{2}\norm{\barSigmaxt^{-1/2}\bXt^\top \bWt}_F^2}
    \paren{\frac{\det(\Sigma)}{\det(\barSigmaxt) } }^{d/2}} \tag{Markov's}\\
    \leq \;& \delta \cdot \prodT \Et\brac{\exp\paren{\frac{1}{2}\norm{\barSigmaxt^{-1/2}\bXt^\top \bWt}_F^2}
    \paren{\frac{\det(\Sigma)}{\det(\barSigmaxt) } }^{d/2}} \tag{Independence} \\
    \leq \;& \delta,
\end{align*}
which by the definition of the event in the first line implies the result of \Cref{prop: multi-task SNM bound}.

==> tex/sufficientID.tex <==


\section{Identifiability Conditions}
We will now make the identifiability condition \eqref{ass:id} more concrete. Identifiability for square loss can often be conveniently expressed as a lower isometric condition relating two $L^2$-norms. We say that \eqref{ass:iso} holds if there exists a constant $\mu>0$ such that:
\begin{align}\label{ass:iso}\tag{\texttt{ISO}}
    \|(f,g)-(f_{0,\star},g_\star)\|_{L^2(\underline{\sfP})}^2 \leq \mu\frac{1}{T}\sum_{t=1}^T \|(f,g)-(f_{0,\star},g_\star)\|_{L^2(\sfP_t)}^2 \qquad \forall f,g\in \scrF\times \scrG. 
\end{align}


\subsection{Nonlinear Representations with Linear Heads}

We impose the following structural assumption in this section. Namely, we suppose that the tuple $(f,g)$ is specified linearly by matrix multiplication:
\begin{align}\label{ass:linheads}\tag{\texttt{LIN}}
    (f,g) (x) = f g(x) \qquad \textnormal{ for every } (f,g)\in \scrF\times \scrG.
\end{align}
Here, we identify $\scrF$ with $\R^{\mathrm{d}_Y \times \mathrm{d}_g}$ so that for each fixed $x\in \sfX$, $g(x)$ is a feature vector in $\R^{\mathrm{d}_g}$. The following is a strengthened version of Lemma 6 in \cite{tripuraneni2020theory} that does not require the covariate marginals to be identical across tasks.

\begin{lemma}\label{lem:lin_id}
Let $F_{0}= f_0 f_0^\top$, $F_\star = \frac{1}{T}\sum_{t=1}^T f_{t,\star} f_{t,\star}^\top$ and suppose $\ker F_\star \subset \ker F_0$. Any model with linear heads of the form \eqref{ass:linheads} satisfying the $\mu$-lower isometry condition \eqref{ass:iso}  also satisfies the identifiability condition \eqref{ass:id} with $\nu^{-1}=\mu\|F_0 F_\star^\dagger \|_{\mathsf{op}}$.
\end{lemma}

\subsubsection{Proof of \Cref{lem:lin_id}}
We begin by writing:
\begin{equation}\label{eq:lin_id_1}
    \begin{aligned}
        &\hspace{-30pt}\inf_{f\in \scrF}\underline{\sfP} \|( f,\widehat g)(X)- Y\|_2^2- \underline{\sfP} \|(f_{0,\star},g_\star)(X)-Y\|_2^2\\
        & \leq \inf_{f\in \scrF}\underline{\sfP} \|( f,\widehat g)(X)-(f_{0,\star},g_\star)(X)\|_2^2 && (f_{0,\star}\textnormal{ is } \underline{\sfP}-\textnormal{optimal})\\
        &\leq  \inf_{f\in \scrF} \frac{\mu}{T}\sum_{t=1}^{T} \sfP_t\|(f,\widehat g)(X)-(f_{0,\star},g_\star)(X)\|_2^2. && \eqref{ass:iso}
    \end{aligned}
\end{equation}
Let $\sfP$ be the uniform mixture over $\sfP_t,t\in [T]$. Define also $\Sigma \triangleq  \sfP \begin{bmatrix} \widehat g(X) \widehat g^\top(X) & \widehat g(X) g_\star^\top (X)\\g_\star(X) \widehat g^\top (X) & g_\star(X) g_\star^\top (X)
\end{bmatrix}$ and the Schur complement $\overline{\Sigma}\triangleq (\sfP  \widehat g(X) \widehat g^\top(X) ) - (\sfP   g_\star(X) \widehat g^\top(X) )(\sfP   g_\star(X) g^\top_\star (X) )^\dagger(\sfP  \widehat g(X)  g^\top_\star(X) )$.


We now rewrite \eqref{eq:lin_id_1} as a single integral by using our definition $\sfP$:
\begin{equation}\label{eq:lin_id_2}
    \begin{aligned}
         &\hspace{-30pt}\inf_{f\in\scrF}\frac{\mu}{T}\sum_{t=1}^{T} \sfP_t\|(f,\widehat g)(X)-(f_{0,\star},g_\star)(X)\|_2^2 \\
         &= \inf_{f\in\scrF}\mu \sfP \|(f,\widehat g)(X)-(f_{0,\star},g_\star)(X)\|_2^2\\
         &=\inf_{f\in\scrF} \mu \begin{bmatrix} f \\ f_0 \end{bmatrix}^\top \Sigma \begin{bmatrix} f \\ f_0 \end{bmatrix} &&(\textnormal{linearity})\\
         &=\mu \tr \left(\overline{\Sigma}f_0f_0^\top \right) &&(\textnormal{optimize over } f)\\
         &=\mu \tr \left(\overline{\Sigma}F_0 \right).
    \end{aligned}
\end{equation}
In a little more detail, the optimization step is a standard calculation about partial minima of quadratic forms \citep[see e.g.][Example 3.15, Appendix A.5.4]{boyd2004convex}.

A similar calcuation reveals that
\begin{align}\label{eq:lin_id_3}
     \frac{1}{ T }\sum_{t=1}^T\inf_{f\in\scrF} \left\{  \Big(\sfP_t  \|(f,\widehat g)(X)- (f_{t,\star},g_\star)(X)\|_2^2\Big)\right\}= \tr \left( \overline{\Sigma}F_\star \right).
\end{align}
Clearly $\mu \tr \left(\overline{\Sigma}F_0\right) \leq  \mu\|F_0 F_\star^\dagger \|_{\mathsf{op}}\tr \left( \overline{\Sigma}F_\star \right)$ and so the result follows by combining \eqref{eq:lin_id_1}, \eqref{eq:lin_id_2} and \eqref{eq:lin_id_3}.
\hfill $\blacksquare$
